Extensive Self-Contrast Enables Feedback-Free Language Model Alignment

Reinforcement learning from human feedback (RLHF) has been a central technique for recent large language model (LLM) alignment. However, its heavy dependence on costly human or LLM-as-Judge preference feedback could stymie its wider applications. In this work, we introduce Self-Contrast, a feedback-free large language model alignment method via exploiting extensive self-generated negatives. With only supervised fine-tuning (SFT) targets, Self-Contrast leverages the LLM itself to generate massive diverse candidates, and harnesses a pre-trained embedding model to filter multiple negatives according to text similarity. Theoretically, we illustrate that in this setting, merely scaling negative responses can still effectively approximate situations with more balanced positive and negative preference annotations. Our experiments with direct preference optimization (DPO) on three datasets show that, Self-Contrast could consistently outperform SFT and standard DPO training by large margins. And as the number of self-generated negatives increases, the performance of Self-Contrast continues to grow. Code and data are available at https://github.com/THUDM/Self-Contrast.

==> figure_with_captions/Compare_with_More_Preference.tex <==
\begin{figure}[htb]
\centering
    \includegraphics[width=8cm]{figures/compare_with_more_pairs_nectar.pdf}
    \caption{Increasing the number of negative samples achieved the same effect as increasing preference data without increasing the number of positive samples.}
\label{fig:Compare_with_More}
\end{figure}

==> figure_with_captions/Compare_with_SPIN.tex <==
\begin{figure}[htb]
\centering
    \includegraphics[width=0.45\columnwidth]{figs/compare-with-spin.pdf}
    \caption{\model achieves higher MT-Bench scores with only SFT prompts, targets, and self-generated negative samples without iterative training compared to previous approaches.}
\label{fig:Compare_with_SPIN}
\vspace{-3mm}
\end{figure}

==> figure_with_captions/HH_Hist.tex <==
\begin{figure}[htb]
\centering
    \includegraphics[width=0.45\columnwidth]{figs/hh-hist.pdf}
    \caption{}
\label{fig:HH_Hist}
\vspace{-3mm}
\end{figure}

==> figure_with_captions/HH_Result.tex <==
\begin{figure}[t]
\centering
% \vspace{-3mm}
    \includegraphics[width=7cm]{figs/negative_sample_quantity_mt_bench_hh.pdf}
    \caption{Win Rate of \model on HH-RLHF. Both implementing response filtering and increasing negative samples benefit performance.}
\label{fig:HH-Result}
\vspace{-3mm}
\end{figure}

==> figure_with_captions/UltraChat-a-Distribution.tex <==
\begin{figure}[t]
\centering
    \includegraphics[width=\columnwidth]{figs/reward-distribution-violin-labeled.pdf}
    \caption{The negative distribution from various response filtering techniques. When $y<1$, it is preferable for the distribution shape to closely resemble the reward model. For $y>1$, lower integral area results in fewer false negatives.}
\vspace{-3mm}
    \label{fig:UltraChat_a_Distribution}
\end{figure}

==> sections/0_abstract.tex <==
Reinforcement learning from human feedback (RLHF) has been a central technique for recent large language model (LLM) alignment.
However, its heavy dependence on human or LLM-as-Judge preference annotations could stymie its wider applications.
In this work, we introduce \model, an annotation-free large language model alignment method via exploiting massive self-generated negatives.
With only supervised fine-tuning (SFT) targets, \model leverages the LLM itself to generate massive candidates, and harnesses a pre-trained embedding model to filter multiple negatives according to text similarity.
Theoretically, we illustrate that as the number of valid negatives approaches infinity, \model will approximate the ideal gradient direction for human preference given certain data distributions.
Our experiments using direct preference optimization (DPO) on two datasets show that, \model could consistently outperform SFT and original DPO by large margins.
And as the number of self-generated negatives increases, the performance \model continues to grow.
Code and data are available at \url{https://github.com/THUDM/Self-Contrast-Alignment}. 


==> sections/7_limitations.tex <==
Although massive negatives and response filtering have proven to be effective, there are still numerous aspects of our approach that require additional investigation. 

\vpara{Assessing human evaluation is necessary.}
To evaluate the human preference, we mainly test our model on MT-Bench and alpaca-eval, which is more likely to the GPT preference. Although the SFT dataset we use is also generated by GPT-4, manual evaluation is still required in actual production to ensure effectiveness.

\vpara{Safety and ethics still need further research.}
Although the positive samples we use come from SFT data, it can ensure a certain level of safety and ethics. However, considering the possibility of false negatives in negative samples, the safety of our training method needs further verification.

\vpara{Stronger embedding model.} A stronger similarity model may lead to more accurate data.
We only filter negative samples with a small pre-trained embedding model based on the response-response relation. However, a stronger or tuned preference embedding model that measures the prompt-response relation, such as \citet{wang2024improving}, may have a more promising feature.

==> sections/multi_negatives_demonstration.tex <==
This section is a proof that massive negatives can play the role of multiple positives.

Supposing the gradient of positive $G_{P}(x, p, n)$ and negative $G_{N}(x, p, n)$ outcomes in a particular solution space are distributed as following:
\begin{flalign}
& G_{P}(x, p, n) \sim N(\mu_{1} ,\sigma_{1}^{2}) \nonumber & \\ 
& G_{N}(x, p, n) \sim N(\mu_{2} ,\sigma_{2}^{2}) \nonumber & \\ 
& c = Cov(G_{P}(x, p, n), G_{N}(x, p, n)) \nonumber & 
\end{flalign}

Because positive samples are usually more similar and negative samples are more diverse, we assume $\sigma_{1} << \sigma_{2}$.

If taking the difference for two signals within a pair: $Grad(x)=G_{P}(x, p, n) - G_{N}(x, p, n)$, then the distribution of this difference can be determined using the properties of the normal distribution:
\begin{flalign}
& Grad(x) \sim N(\mu_{1}-\mu_{2} ,\sigma_{1}^{2}+\sigma_{2}^{2}+2c) &
\end{flalign}

Now, if we repeat the above process $l$ times, sampling a positive and a negative response each time, we will obtain $l$ samples of $Grad(x)$. According to the Central Limit Theorem, the sample mean of these differences will approach a normal distribution:
\begin{flalign}
& \overline{Grad(x)_{l}} \sim N(\mu_{1}-\mu_{2} ,\frac{1}{l}(\sigma_{1}^{2}+\sigma_{2}^{2}+2c)) &
\end{flalign}

On the contrary, we define another difference based on a self-contrast strategy, denoted as $Grad(x)_{self-contrast}$  which has the same initial distribution as $Grad(x)$.
$Grad(x)_{self-contrast}=G_{P}(x, p, n) - G_{N}(x, p, n)$.
With the new sampling strategy where we independently sample $k=1$ positives and $m$ negatives for each positive to create new difference samples, thus obtaining $m \times k$ total samples. The mean of these samples will also follow a normal distribution by the Central Limit Theorem:
\begin{multline}
\overline{Grad(x)_{self-contrast_{m}}} \\ \sim N(\mu_{1}-\mu_{2} ,\frac{1}{k}(\sigma_{1}^{2}+\frac{\sigma_{2}^{2}}{m}+2c))
\end{multline}

For the traditional and Self-Contrast methods, the $1-\alpha$ confidence intervals are expressed as follows:
\begin{flalign}
& RNG_{l}=2\cdot z\cdot\sqrt{\frac{1}{l}(\sigma_{1}^{2}+\sigma_{2}^{2}+2c}) &\\
& RNG_{m}=2\cdot z\cdot \sqrt{\frac{1}{k}(\sigma_{1}^{2}+\frac{\sigma_{2}^{2}}{m}+2c)} &
\end{flalign}

Where $z$ represents the standard normal distribution's $z$-score corresponding to a confidence level $1-\alpha$ of $95\%$, commonly accepted as 1.96.

Supposing $\beta=\frac{k}{l}$ that represents the ratio of possitive samples needed for self-contrast against the traditional methods, $\lambda=\frac{\sigma_{2}^{2}}{\sigma_{1}^{2}+\sigma_{2}^{2}+2c}$ determined by the solution space. To ensure $RNG_{m} < RNG_{l}$, $m$ must be large enough which equates to:
\begin{flalign}
& \beta > 1 + \lambda(\frac{1}{m}-1)&
\end{flalign}

In our cases where $\beta=\frac{1}{l}$, there is a solution for $m$ when $l<\frac{1}{1-\lambda}$:
\begin{flalign}
\label{M-L-Ralation}
& m > \frac{\lambda}{\lambda + (\frac{1}{l} - 1)} &
\end{flalign}

